3D Weak Gravitational Lensing of the CMB and Galaxies

In this paper we present a power spectrum formalism that combines the full three-dimensional information from the galaxy ellipticity field, with information from the cosmic microwave background (CMB). We include in this approach galaxy cosmic shear and galaxy intrinsic alignments, CMB deflection, CMB temperature and CMB polarisation data; including the inter-datum power spectra between all quantities. We apply this to forecasting cosmological parameter errors for CMB and imaging surveys for Euclid-like, Planck, ACTPoL, and CoRE-like experiments. We show that the additional covariance between the CMB and ellipticity measurements can improve dark energy equation of state measurements by 15%, and the combination of cosmic shear and the CMB, from Euclid-like and CoRE-like experiments, could in principle measure the sum of neutrino masses with an error of 0.003 eV.

==> abstract <==
In this paper we present a power spectrum formalism that combines the full three-dimensional information from the galaxy ellipticity field, with information from the cosmic microwave background (CMB). We include in this approach galaxy cosmic shear and galaxy intrinsic alignments, CMB deflection, CMB temperature and CMB polarisation data; including the inter-datum power spectra between all quantities. We apply this to forecasting cosmological parameter errors for CMB and imaging surveys for Euclid-like, Planck, ACTPoL, and CoRE-like experiments. We show that the additional covariance between the CMB and ellipticity measurements can improve dark energy equation of state measurements by 15\%, and the combination of cosmic shear and the CMB, from Euclid-like and CoRE-like experiments, could in principle measure the sum of neutrino masses with an error of $0.003$ eV.
